Explanation Regularisation through the Lens of Attributions

Explanation regularisation (ER) has been introduced as a way to guide text classifiers to form their predictions relying on input tokens that humans consider plausible. This is achieved by introducing an auxiliary explanation loss that measures how well the output of an input attribution technique for the model agrees with human-annotated rationales. The guidance appears to benefit performance in out-of-domain (OOD) settings, presumably due to an increased reliance on "plausible" tokens. However, previous work has under-explored the impact of guidance on that reliance, particularly when reliance is measured using attribution techniques different from those used to guide the model. In this work, we seek to close this gap, and also explore the relationship between reliance on plausible features and OOD performance. We find that the connection between ER and the ability of a classifier to rely on plausible features has been overstated and that a stronger reliance on plausible tokens does not seem to be the cause for OOD improvements.

==> figures/sa_suff_comp.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{1.\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/suff_comp_sufficiency.pdf}
        \caption{Normalised Sufficiency}
        \label{subfig:sa_attributions_correlations_kendall}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{1.\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/suff_comp_comprehensiveness.pdf}
        \caption{Normalised Comprehensiveness}
        \label{subfig:sa_attributions_correlations_pearson}
    \end{subfigure}
\caption{Normalised sufficiency and comprehensiveness ($\uparrow$) scores for the top 1\%, 5\%, 10\%, 20\%, and 50\% tokens according to a given attribution technique, for SST-Dev.}
\label{fig:sa_suff_comp}
\end{figure*}

